Dynamic Prompting: A Unified Framework for Prompt Tuning

It has been demonstrated that the art of prompt tuning is highly effective in efficiently extracting knowledge from pretrained foundation models, encompassing pretrained language models (PLMs), vision pretrained models, and vision-language (V-L) models. However, the efficacy of employing fixed soft prompts with a predetermined position for concatenation with inputs for all instances, irrespective of their inherent disparities, remains uncertain. Variables such as the position, length, and representations of prompts across diverse instances and tasks can substantially influence the performance of prompt tuning. In this context, we provide a theoretical analysis, which reveals that optimizing the position of the prompt to encompass the input can capture additional semantic information that traditional prefix or postfix prompt tuning methods fail to capture. Building upon our analysis, we present a unified dynamic prompt (DP) tuning strategy that dynamically determines different factors of prompts based on specific tasks and instances. To accomplish this, we employ a lightweight learning network with Gumble-Softmax, allowing us to learn instance-dependent guidance. Experimental results underscore the significant performance improvement achieved by dynamic prompt tuning across a wide range of tasks, including NLP tasks, vision recognition tasks, and vision-language tasks. Furthermore, we establish the universal applicability of our approach under full-data, few-shot, and multitask scenarios. Codes are available at https://github.com/Xianjun-Yang/DPT.

==> sections/s1_intro.tex <==

\section{Introduction}
The release of ChatGPT \cite{GPT35} and GPT-4 \cite{openai2023gpt} by OpenAI has sparked global discussions on the effective utilization of AI-assistant writing. Despite the success, they have also given rise to various challenges such as fake news \cite{zellers2019defending} and technology-aided plagiarism \cite{bommasani2021opportunities}. There have been instances where AI-generated scientific abstracts have managed to deceive scientists \cite{gao2022comparing, Else2023AbstractsWB}, leading to a disruption in trust towards scientific knowledge. Unfortunately, the progress in detecting AI-generated text lags behind the rapid advancement of AI itself.

As AI-generated text approaches high quality, effectively detecting such text presents fundamental difficulties. This has led to a recent debate on the detectability of AI-generated text \cite{chakraborty2023possibilities, krishna2023paraphrasing, sadasivan2023can}. Nevertheless, there is still a lack of practical methodology for AI-generated text detection, particularly in the era of ChatGPT. We aim to present a general, explainable, and robust detection method for LLMs, especially as these models continue to improve. Some existing detection methods utilize perturbation-based approaches like DetectGPT \cite{mitchell2023detectgpt} or rank/entropy-based methods \cite{gehrmann-etal-2019-gltr, solaiman2019release, ippolito-etal-2020-automatic}. However, these detection tools fail when the token probability is not provided, as is the case with the OpenAI's \texttt{GPT-3.5} series. Furthermore, the lack of details about how those most potent language models are developed poses an additional challenge in detecting them. This challenge will continue to escalate as these LLMs undergo continuous updates and advancements.

Hence, there is a pressing demand to effectively detect GPT-generated text to match the rapid advancements of LLMs. Moreover, when formulating the detection methodology, an essential focus lies on explainability, an aspect that is often absent in existing methods that solely provide a prediction devoid of supporting evidence. This aspect holds significant importance, especially in education, as it poses challenges for educators in comprehending the rationale behind specific decisions. %As such, an effective detection strategy that is able to provide explainable evidence is desirable for making GPT-generated text detection a practical solution.

In this study, we address two scenarios in Figure \ref{fig:pipeline}: 1) White-box detection, where access to the model output token probability is available, and 2) Black-box detection, where such access is unavailable. This allows us to cater to both cases and provide comprehensive solutions. Our work builds upon the observation that LLMs tend to decode repetitive $n$-grams as the previous run of generations given an appropriate preceding text. On the contrary, human-written text tends to have a lower probability of being decoded by the language models. We also theoretically analyze the possibility of AI-generated text in terms of true positive rate (TPR) and false positive rate (FPR), which is orthogonal to the current debate about detectability \cite{sadasivan2023can, chakraborty2023possibilities}.
%This opacity can erode trust in the system, as users may hesitate to rely on the output of a machine-learning model they cannot interpret.
To sum up, our contributions are as follows:
\begin{itemize}
\item We have developed zero-shot detection algorithms for texts generated by GPT models in both black-box and white-box scenarios and validated the effectiveness using the five most advanced LLMs on five datasets.
%Our solutions are training-free and offer the capability to provide explainable evidence, making them highly practical for real-world usage.
\item We conduct extensive experiments to demonstrate its superiority over previous training-based baselines and validate its robustness on non-English, or revised text attacks and provide the capability for model sourcing.
%in various situations. The outcomes show that our technique performs significantly better than the state-of-the-art (SOTA) baselines.
\item We additionally provide explainable evidence for detection decisions and analyze the detectability of AI-generated text in terms of TPR and FPR rather than AUROC on the debate of detection possibility.
%, theoretically which may be of independent interest.
% utilizing binary hypothesis testing,
\end{itemize}

\begin{figure*}[t!]\vspace{-0.5cm}
  \centering
  \includegraphics[width=0.95\linewidth]{figure/overall_fig.pdf}
  \caption{Overview of our framework. Given a candidate passage \textit{x}, we aim to distinguish whether it is generated by a certain language model like \texttt{GPT-3.5-turbo} or human. Our method first truncates the original passage by a ratio to obtain the truncated text $x'$ and remaining text $y_0$, then $x'$ is fed into the language model for generating \textit{K} new outputs $\{y_1, ..., y_K \}$. Finally, a \textit{BScore} or \textit{WScore} between the new outputs and $y_0$ is calculated for classifying original candidate \textit{x} into human or AI-generated content. The threshold $\epsilon$ balances TPR and FPR. This example is taken from the PubMedQA dataset. }\vspace{-0.2cm}
  \label{fig:pipeline}
\end{figure*}

% https://openai.com/brand#mark-usage-terms

==> sections/s2_related_work.tex <==
\section{Related Work}

\stitle{Large Language Models.} The recent development of large foundation language models \cite{bommasani2021opportunities} has revolutionized the field of natural language processing (NLP) and generated significant interest among researchers and practitioners. 
%These models, trained on massive amounts of text data, have demonstrated remarkable capabilities in generating highly coherent and contextually accurate text.
The large language models are usually built on the transformer \cite{vaswani2017attention} architecture, including encoder-only BERT \cite{devlin-etal-2019-bert}, encoder plus decoder T5 \cite{raffel2020exploring}, and decoder-only GPT-2 \cite{radford2019language}. %These models laid the foundation for the current generation of highly advanced models. 
And the success of instruction-tuned GPT-3 \cite{brown2020language} and ChatGPT \cite{schulman2022chatgpt} has garnered attention for the zero-shot ability of GPT to generate text that is of high quality and often indistinguishable from human-written content. Following the success of GPT, most advanced models usually adopt the decoder-only design, like Google's LaMDA \cite{thoppilan2022lamda}, Meta's OPT \cite{zhang2022opt}, LLaMa \cite{touvron2023llama} and OpenAI's GPT-4 \cite{openai2023gpt}.
Those models are typically trained on vast amounts of text data using self-supervised learning by predicting the next word in a sentence and then are fine-tuned on specific instructions to align with human preference \cite{ouyang2022training}. During generation, beam search is widely used in conjunction with top-$k$ sampling \cite{fan-etal-2018-hierarchical} and nucleus sampling \cite{holtzmancurious}. 
Despite being powerful, the growing prevalence of AI has raised various ethical concerns, including fake news \cite{zellers2019defending} and homework plagiarism \cite{stokel2022ai}. This has led to increased interest in developing effective methods for detecting AI-generated text \cite{chen2023gpt, zhan2023g3detector, li2023deepfake, yu2023gpt, verma2023ghostbuster, wu2023llmdet, wang2023m4} or online chatbot \cite{wang2023bot}. 

\stitle{Detecting AI-generated Text.} The earlier work focused on feature-based methods like extracting linguistic features %, such as syntax, semantics, and word frequency, 
from text to identify AI-generated content, including the frequency of rare bigrams \cite{grechnikov2009detection}, $n$-gram frequencies \cite{badaskar2008identifying}, or top-$k$ words in GLTR \cite{gehrmann-etal-2019-gltr} under the assumption that generated words come from a max head distribution. 
However, this has become a significant concern in cases where language models with advanced generation capabilities, such as ChatGPT, produce lengthy text that is exceedingly difficult to differentiate even for human evaluators. Then some researchers have employed fine-tuned language models to identify AI-generated text. For example, OpenAI trained an OpenAI Text Classifier \cite{AITextClassifier} on a collection of millions of text. GPTZero \cite{GPTZero} was developed based on the difference between the perplexity score of text. 
However, training-based methods still do not generalize well and are even biased towards non-native writers \cite{liang2023gpt}. More importantly, the detector model has to be trained periodically to catch up with the release of new LLMs updates since they are being actively updated. 
Another category falls into the training-free paradigm, and DetectGPT \cite{mitchell2023detectgpt} is a zero-shot method that utilizes the observation that machine-generated passages occupy regions with clear negative log probability curvature. And \cite{kirchenbauer2023watermark} developed watermarks for language modeling by adding a green list of tokens during sampling.
While these methods have demonstrated varying levels of success, our proposed \methodname~ offers a unique and effective way of identifying GPT-generated text by exploiting the inherent differences in text continuation patterns between human and AI-generated content. Compared with the classifier-only detector, our method also provides evidence for detection results and thus is explainable.

==> sections/s3_method.tex <==
\section{Methodology}
Inspired by the fact that DNA (deoxyribonucleic acid) is unique for every organism, we assume every individual pre-trained LLM also has its unique DNA for being identified.

% \textbf{Assumption 1.} \textit{An AI model and a human tends to write different continuing text given a preceding text. And so does different AI models. }

\textbf{Assumption.} \textit{Each AI model possesses its distinctive DNA, which may manifest either in its inclination towards generating comparable n-grams or in the shape of its probability curve. }

\stitle{Task Definition.} We formulate the detection as a binary classification task. Given a text sequence $S$, and a specific language model $LM$ like \texttt{GPT-4}, the goal is to classify whether $S$ is generated by the $LM$ or written by humans. In the black-box setting, we only have access to the output text generated by the $LM$ by arbitrary input, while in the white-box setting, we additionally have access to the model output probability for each token. %Since our method is training-free, we do not have a large collection consisting of human and machine-generated text, which is usually in the million-level in previous work like OpenAI detector or GPTZero. 
Formally, given a sequence $S = [s_i, ..., s_L]$, where $L$ is the sequence length, we define a truncate rate $\gamma$ for splitting the sequence into two parts: $S_1 = [s_1, ..., s_{\lceil \gamma L \rceil}]$, and $S_2 = [s_{ \lceil \gamma L \rceil + 1}, ..., s_L]$. Next, we ask the LLMs to continue generating the remaining sequences purely based on $S_1$, and the generated results are denoted by $S' = LM(S_1)$. In practice, we sample the new results for $K$ times to get a set of sequences $\Omega = \{S'_1, ..., S'_k, ..., S'_K \}$. Then we can have a training-free classifier on the similarities between $\Omega$ and $S_2$. The classifier will output a scoring value used for classification based on some threshold, which balances the FPR and TPR. The overall pipeline is elaborated in Figure \ref{fig:pipeline}, and we will dive into the details in the following.

\subsection{Black-box Detection}
Our main focus is on black-box detection since there is an increasing trend for large tech companies like Google and OpenAI to make the details of their chatbot Bard and ChatGPT closed. In real-world scenarios, users typically can only interact with AI through API and have no access to the token probability, not to mention the underlying model weights. Thus, in the black-box scenario, we do not rely on any information about the model parameters except for the textual input and outputs. 

Armed with the model outputs $\Omega$ and $S_2$, we compare their $n$-gram similarity to distinguish human- and GPT-written text. Based on our assumption, the human-generated $S_2$ will have a much lower overlap with $\Omega$, compared with GPT-generated text. We define the \methodname~ \textit{BScore}:
\begin{equation*}
%\begin{aligned}
BScore(S, \Omega) =  \frac{1}{K} \sum\limits_{k=1}^{K} \sum\limits_{n=n_{0}}^{N}  f(n)  \frac{|n{-}grams(S'_k)  \cap n{-}grams(S_2) |}{ |S'_k|  |n {-} grams(S_2) |},
%\end{aligned}
\end{equation*}\label{eq:black}

where $f(n)$ is a weight function for different $n{-}grams$. $|S'_k|$ is used for length normalization.
In practice, we set $f(n){=}n\log(n)$, $n_0{=}4, N{=}25$ and find it works well across all datasets and models. More comparisons on parameter sensitivity can be found in Appendix \ref{app:parameter}.
%issue: length normalized, model unknown? prefix text?


\subsection{White-box Detection}
In the white-box detection, we only have additional access to the model output probabilities on the input and the generated tokens, while model weights and token probabilities over the whole vocabulary are still unknown. This service is supported by OpenAI's \texttt{text-davinci-003} but is no longer supported since the \texttt{GPT-3.5} series. 
%For open-accessed models like \texttt{GPT-NeoX-20B}, we also limit ourselves to accessing only the output token probabilities, making it fair with \texttt{text-davinci-003}. 
Inspired by the assumption of the unique probability curve, we can also calculate a \methodname~ \textit{WScore} between $\Omega$ and $S_2$:

\begin{equation*}
\begin{aligned}
WScore(S, \Omega) = \frac{1}{K} \sum\limits_{k=1}^{K} log \frac{p(S_2|S_1)}{p(S'_k|S_1)}. 
\end{aligned}
\end{equation*}

In both the black-box and white-box settings, two parameters play a critical role in determining the detection accuracy: the truncation ratio ($\gamma$) and the number of re-prompting iterations ($K$).

\subsection{Evidence}\label{evidence}
One additional benefit of our method is to provide an explanation of our detection results, compared with only Yes or No answers. 
We define the evidence $\mathcal{E}$ as some overlapped sentence-piece between each re-generated text in $\Omega$ and $S_2$. 
\begin{equation*}
%\begin{aligned}
\mathcal{E} = \bigcup\limits_{k=1}^{K}  \{ piece_{k_1} \in S'_k, ..., piece_{k_M} \in S'_k  \},
%\end{aligned}
\end{equation*}
where $piece_{k_m}$ in $S'_k$ is assumed to be evidence if their corresponding $n{-}gram|_{n=m}$ matches within $S_2$. When $n$ is large, the sentence pieces serve as strong evidence for AI-generated text since human tends to write dissimilar texts. It is important to note that despite substantial evidence, there remains a possibility of misclassification. We highly recommend utilizing the evidence in a flexible manner, particularly when evaluating student plagiarism. Defining the precise boundaries of what constitutes plagiarism is a complex matter, and we defer more exploration to future research endeavors.  


==> sections/s4_experiments.tex <==
\section{Experiments}

\subsection{On the Datasets for Detection}\label{sec:Memorization}
\textbf{Model Memorization.} Previous research \cite{carlini2021extracting} has demonstrated the ability to extract numerous verbatim text sequences from the training data on LLMs, employing appropriate prompting techniques. This finding has received further validation through recent work \cite{yu2023bag}, where enhanced strategies for extracting training data are introduced. Consequently, when the generated text is verbatim copying of the training data, it becomes indistinguishable from human-written text, rendering the distinction between AI-generated and human-written text futile. To investigate this aspect, we evaluate the widely adopted open-end generation WikiText-103 dataset \cite{meritypointer}, which originated from Wikipedia and has been extensively utilized for training subsequent models. Through our experiments, we discovered that the \texttt{text-davinci-003} model tends to memorize the context and generate text that closely resembles the original data. Specifically, out of 100 examples randomly selected from the validation split, 13 prompt outputs exhibited identical continuous tokens spanning three consecutive sentences, as detailed in Appendix \ref{app:parameter}. This phenomenon poses a challenge in distinguishing these instances as AI-generated rather than human-written text. Consequently, we argue that careful consideration must be given to the choice of the dataset when testing detectors.

\textbf{What Makes a Dataset Good for AI Detection?} %As mentioned earlier, when selecting a dataset for detection purposes, it is crucial to ensure that the model does not generate verbatim copies from the training data. 
Essentially, along with common requirements such as \texttt{Quality}, \texttt{Accessibility}, \texttt{Legal compliance}, \texttt{Diversity}, \texttt{Size}, and others, we suggest three additional criteria: 1) The text should have a moderate length, typically exceeding 1000 characters, as the OpenAI classifier only accepts text longer than this threshold. Short answers are significantly more difficult to be differentiated. 2) The dataset should be relatively new and not yet extensively used for training the most up-to-date LLMs, ensuring the evaluation of models on unseen data. 3) The length of text samples from both humans and AI should be comparable to enable a fair comparison. For instance, in experiments conducted by \cite{krishna2023paraphrasing}, both the AI-generated and human-written texts were limited to approximately 300 tokens. In our study, we adopt a similar setup.

\subsection{Experimental Setup}
\textbf{Five Datasets.} To prevent LLMs from verbatim copying from training data, we collected two newest datasets. One is the Reddit long-form question-answer dataset from the ELI5 community \cite{fan-etal-2019-eli5}\footnote{\url{https://www.reddit.com/r/explainlikeimfive/}}. We filtered the data based on physics and biology flairs, focusing on the period from January 2022 to March 2023\footnote{Although OpenAI \cite{openai2023gpt} claimed training data is truncated up to September 2021, their model may encounter data beyond this date during alignment, our filtering reduces the potential for cheating as OpenAI has not disclosed its data usage specifics.}. We also acquired scientific abstracts published on the Nature website on April 23, 2023, and performed our experiments on the same day to minimize the possibility of OpenAI utilizing the data for model updates. Furthermore, we utilized publicly available datasets such as PubMedQA \cite{jin-etal-2019-pubmedqa} to showcase the effectiveness in the biomedical domain. For evaluating the detection of fake news, we used the Xsum \cite{narayan-etal-2018-dont} dataset and prompted the model with the first two sentences. For non-English text, we utilized the English and German splits of WMT16 \cite{bojar2016findings}. Specifically, we filtered German sentences of approximately 200 words and prompted the model with the first 20 words for generation. Although these datasets may have been employed for training and updating existing AI products, we leveraged them responsibly to support our research findings. We use 150 to 200 instances from each dataset for testing and more details are in Appendix \ref{app:parameter}.


\textbf{Five Models.} First, we include the three most advanced LLMs from OpenAI API \footnote{https://platform.openai.com/docs/api-reference}: GPT-3 (\texttt{text-davinci-003}), ChatGPT (\texttt{gpt-3.5-turbo}), and GPT-4 (\texttt{gpt-4-0314}). Among these, only \texttt{text-davinci-003} provides access to the top-5 token probability. Notably, the \texttt{gpt-3.5-turbo} model is frequently updated by the OpenAI team, while \texttt{gpt-4-0314} remains frozen during our testing. As the \texttt{gpt-3.5-turbo} model tends to demonstrate increased result inconsistency over time due to these updates, our objective is to assess its detection capability under such evolving circumstances.
In addition to the closed models from OpenAI, we also incorporate two open-sourced language models based on the GPT architecture: LLaMa-13B \cite{touvron2023llama} and GPT-NeoX-20B \cite{black2022gpt}. Unless explicitly stated, we employ a temperature of $0.7$ to strike a balance between text diversity and quality for all five models, as has been done in previous research \cite{krishna2023paraphrasing}. All other parameters remain at their default values, with the exception of a maximum token length of 300.
%\footnote{We conduct our experiments using four Nvidia A40 48G GPUs with half precision.}

\textbf{Two Metrics.} Previous studies \cite{mitchell2023detectgpt, sadasivan2023can} have primarily focused on utilizing the Area Under The ROC Curve (AUROC) score for evaluating detection algorithm effectiveness. However, our research indicates that this metric may not always offer an accurate assessment, particularly when the AUROC score approaches the ideal upper bound of 1.0. Notably, two detectors with an identical AUROC score of $0.99$ can demonstrate significant disparities in user experience in terms of detection quality.
To ensure the reliability of detection methods for real-life deployment, it is crucial to maintain a high TPR while minimizing the FPR. Therefore, we also present TPR scores at a fixed 1\% FPR, as in \cite{krishna2023paraphrasing}.

\textbf{Two Algorithms.} For models like \texttt{GPT-3.5} and \texttt{GPT-4} without disclosing any token probability, we employ the black-box detection algorithm and solely provide results based on \textit{BScore}. Conversely, for \texttt{text-davinci-003}, \texttt{GPT-NeoX-20B}, and \texttt{LLaMa-13B} with access to token probability, we could additionally provide white-box detection results using \textit{WScore}.

\textbf{Three Baselines.} We consider two strong supervised training-based baselines: GPTZero \cite{GPTZero} and OpenAI's classifier \cite{AITextClassifier}. Although detailed information about the internal workings of these classifiers is not provided, certain key aspects have been disclosed. GPTZero is trained to assess perplexity and burstiness in text, enabling it to distinguish between artificially generated and human-crafted content. On the other hand, OpenAI's classifier is fine-tuned from a collection of 34 models from five different organizations. We also consider DetectGPT \cite{mitchell2023detectgpt} for \texttt{text-davinci-003} since it relies on the token probability for detection. %But it requires at least 100 perturbations to achieve good performance, so we only test it on two datasets due to budget constraints.
Notably, previous entropy \cite{gehrmann-etal-2019-gltr} or rank-based algorithms \cite{solaiman2019release, ippolito-etal-2020-automatic} are excluded from comparison as they rely on token probabilities over the whole vocabulary, which is not available in ChatGPT's era. 

\textbf{Two Detection Scenarios.} When detecting AI-generated text, two realistic scenarios arise: the prompt used for generation is either known or unknown to the detector. For instance, in the case of questions and answers on Reddit, the prompts are typically known. Conversely, when generating fake news, the prompts are usually unknown. In our experiments, we evaluate both scenarios to replicate real-world conditions. Besides, there could be more complicated system prompt and smart prompt attacks, and we leave the exploration in Appendix \ref{app:parameter}. 

%It is worth noting that there could also be a potential smart prompt attack, wherein the known question is prompted with additional smart instructions. However, addressing such attacks falls outside the scope of our current work. 




==> sections/s5_results.tex <==
\vspace{-0.1cm}
\section{Results and Analysis}
\vspace{-0.1cm}

\input{tables/table-overall}

\stitle{Overall Results.} The overall results are presented in Table \ref{tab:overall}. Our zero-shot detector consistently achieves superior performance compared to the supervised baselines, namely GPTZero \cite{GPTZero} and OpenAI's Classifier \cite{AITextClassifier}, in terms of both AUROC and TPR. Notably, our black-box detector exhibits enhanced results when provided with the golden question prompt, although intriguingly, optimal performance is sometimes achieved without utilizing a golden prompt.
Another noteworthy observation is the significant underperformance of GPTZero, and OpenAI's Classifier on outputs generated from our newly curated datasets, namely Reddit-ELI5 and Scientific abstracts, in contrast to the established datasets, PubMedQA and Xsum. This disparity can be attributed to the limited training data, highlighting the vulnerability of training-based classifiers. Conversely, our \methodname~ consistently exhibits exceptional performance across both historical and newest datasets.
Additionally, our detector excels DetectGPT by a large margin under the white-box setting with even fewer costs. It is imperative to acknowledge that a considerable number of technology companies have ceased the disclosure of token probability, rendering this type of white-box detection less feasible from the user's perspective in actual world situations. Nevertheless, we posit that it remains viable for the providers of LLMs service to implement these in-house detection systems on their end.


\stitle{Truncation Ratio.} The first question to our \methodname~ pertains to the optimal truncation ratio for achieving good performance. In order to address this query, we conducted a series of experiments using two models on three distinct datasets: the Reddit dataset using \texttt{gpt-3.5-turbo} with known prompts, PubMedQA using \texttt{gpt-3.5-turbo} without known prompts, and the Xsum dataset using \texttt{LLaMa-13B} without golden prompts. Each dataset comprised 150-200 instances. The truncation ratio $\gamma$ was systematically varied across values of $\{0.02, 0.1, 0.3, 0.5, 0.7, 0.9, 0.98\}$. The obtained results are illustrated in Figure \ref{fig:truncation}. It becomes evident that the overall detection performance initially exhibits an upward trend, followed by a subsequent decline. Intuitively, when presented with a very brief prompt, the model possesses a greater degree of freedom to generate diverse text. Conversely, imposing severe constraints by incorporating almost the entire original text severely restricts the space for text generation. Consequently, the most favorable truncation ratio is expected to fall within the middle range. Our investigations revealed that a truncation ratio of $0.5$ consistently yielded favorable outcomes across all considered models and datasets. Notice that this might be unsuitable for a longer text that starts with AI-generated prefix text and is followed by human-written text, and we argue that it is possible to apply a sliding window to do the detection. Due to the complexity of such scenarios, we leave the discussion in Appendix \ref{app:parameter}.
\input{tables/truncatio}

\stitle{Number of Re-generations.} In order to investigate the optimal number of re-generations required to achieve satisfactory detection results, a series of experiments was conducted using \methodname~ on four distinct datasets. The results obtained from these experiments are visualized in Figure \ref{fig:auroc_tpr}.
In terms of the AUROC score, it is evident that employing either 10(black-box) or 5(white-box) re-prompting instances is sufficient to reach a saturation point. On the other hand, the TPR metric exhibits continuous improvement until approximately five re-generations, regardless of whether the black-box or white-box setting is utilized.
Considering the costs of invoking OpenAI's API, we assert that a range of 5-10 re-generations represents a reasonable choice to ensure desired performance.
\input{tables/auroc_regen}

\stitle{Decoding Temperature.} \textit{Temperature}\footnote{https://platform.openai.com/docs/api-reference/chat/create\#chat/create-temperature} \textit{T} controls the randomness during generation to trade off text quality and diversity \cite{DBLP:conf/icml/NaeemOUCY20}. In general, higher \textit{T} will make the output more random, while lower \textit{T} will make it more focused and deterministic.
To explore how different classifiers work when the temperature varies, we tried a \textit{T} range of $\{ 0.7, 1.0, 1.4, 1.8\}$ on the Reddit dataset. However, we discarded $\textit{T}{=}1.8$ since we discovered that it resulted in nonsensical text. We depicted the changes in Figure \ref{fig:temperature}.
\sloppy
\begin{wrapfigure}{l}{0.63\textwidth}\vspace{-0.3cm}
\includegraphics[width=0.63\textwidth]{figure/temperature.pdf}
\caption{ The impact of decoding temperature on detection performance, conducted using \texttt{gpt-3.5-turbo}. }%\vspace{-0.4cm}
\vspace{-0.4cm}
\label{fig:temperature}
\end{wrapfigure}
Surprisingly, we found that training-based methods like GPTZero and OpenAI's classifier drop the performance significantly. Although they both claimed to train the detector on millions of texts, no detailed information is disclosed about how they got the GPT-generated text. The results show these methods are very sensitive to the decoding \textit{T}. But ours consistently outperforms those two baselines, although also demonstrating a drop in AUROC and more decrease in TPR.
% \input{tables/temperature}

\stitle{Revised Text.}\label{res:revise} In practical applications, AI-generated text often undergoes revision either by another language model or by human users themselves. In such cases, it is crucial to assess the robustness of an AI detector. Taking inspiration from DetectGPT \cite{mitchell2023detectgpt}, who made use of the mask-filling capability of T5-3B \cite{raffel2020exploring}, we also simulate human revisions by randomly replacing a fraction of $r\%$ of 5-word spans in 100 instances from the Reddit dataset answered by \texttt{GPT-4}. and employ the \texttt{T5-3B} model to fill in the masks. We experiment with various revision ratios, specifically $r\% {\in} \{ 0.0, 0.1, 0.2, 0.35, 0.5 \}$, and present the results in Figure \ref{fig:revise_ratio}. It is evident that GPTZero and OpenAI's classifier both experience a slight decline in performance with moderate revision ratios, but their performances dramatically deteriorate when the text is heavily revised ($r\% > 0.3$). In contrast, our proposed method consistently outperforms both classifiers and maintains a stable detection performance. Even when approximately half of the text has been revised, our \methodname~ shows only a slight drop in AUROC from 99.09 to 98.48, indicating its robustness in detecting revised text.

\stitle{Non-English Detection.} Prior detection tools, primarily designed for English, have often overlooked the need for non-English detection. A recent study discovered that many AI classifiers tend to exhibit bias against non-native English writers \cite{liang2023gpt}, which further underscores the importance of focusing on other languages. We selected the English and German splits of WMT-2016 to evaluate performance in German and tested our white-box detection on \texttt{text-davinci-003} and black-box detection on \texttt{ GPT-turbo-35}. The results are depicted in Figure \ref{fig:german}. 
It is apparent that GPTZero performs poorly, as it is no better than random guessing, suggesting a lack of German training data.  Compared to OpenAI's supervised classifier, our zero-shot methods achieve comparable or even superior results, demonstrating its robustness in non-English text. 
\input{tables/german}

\stitle{Explainability} One main advantage of our detection method is to provide not only a YES or NO detection decision but also reasonable explanations, as discussed in Sec. \ref{evidence}
The explainability of detectors can significantly enhance their effectiveness and utility. We illustrate one example of evidence in Figure \ref{fig:pipeline}. As we can see, out of 20 re-generations, we found three cases where there is a large portion of identical phases, starting and ending differently, though. Those non-trivial N-gram overlaps provide strong evidence to support our claim that the candidate text $x$ is written by AI rather than humans. Such explainability is crucial for educators to find evidence of plagiarism, which can not be achieved by a binary classifier like OpenAI's detector.
More complete examples can be found in Appendix \ref{app:Explainability} due to the space limit. 


\stitle{Open-Sourced Models.} Despite the proprietary nature of OpenAI's LLMs, we have also evaluated the effectiveness of \methodname~ using two large, open-source language models: \texttt{GPT-NeoX-20B} and \texttt{LLaMa-13B}, both employing a transformer decoder-only architecture. We replicated the same experimental setup on the Reddit and Xsum datasets, with results presented in Table \ref{tab:gptx}. 
We observed a significant performance degradation on two training-based classifiers, namely GPTZero and OpenAI's classifier, across the selected datasets and models. This outcome could potentially be attributed to the scarcity of training data from these two models, which in turn exposes the vulnerabilities of training-based detectors when applied to newly developed models. 
Contrarily, our methods consistently outperformed baselines across different models and corpora under both black- and white-box settings, irrespective of the availability of the golden prompt. Given the continuous release of new models to the public, maintaining classifier robustness towards these emerging models is of paramount importance. We hope our \methodname~ offers a viable solution to this pressing issue.
\input{tables/gptx}

\stitle{Model Sourcing.} Despite distinguishing text from AI or humans, one auxiliary utility of our work is that it can be applied to a novel task that we named \textit{Model Sourcing}: detection of which model the text is generated from, assuming each model possesses their unique DNA. For example, given the candidate text and candidate models $\{\texttt{GPT-3.5-turbo}, \texttt{LLaMa-13B}, \texttt{GPT-NeoX-20B}, \texttt{GPT-4}\}$, we would like to know which model the text most likely comes from. Concurrently, \cite{li2023origin} proposed origin tracking, referring to a similar meaning.  
Our method works by performing the same truncation-then-regeneration pipeline and ranks the result to identify the model source. 
For simplicity, we test this idea by using combinations of these candidate models on the Reddit and Xsum datasets, as shown in Table \ref{tab:modelsouring}. Notice that this task can not be solved by previous AI detectors that only distinguish between humans and machines. More broadly, model sourcing can be used when we do not know which model the text might be generated from. 

\stitle{Possibility of Detection.}
Previous debate \cite{ sadasivan2023can} draws insights from the binary hypothesis test and LeCam's lemma \citep{le2012asymptotic,wasserman2013}, and states that for any text distributions of human $m$ and machine $h$, detector $\texttt{AUROC} \leq \frac{1}{2} {+} \texttt{TV} (m, h) {-} \frac{\texttt{TV} (m, h)^2}{2}$ and this upper bound led to the claim of impossibility when Total Variance $\texttt{TV} (m, h)$ is approaching $0$. However, \cite{chakraborty2023possibilities} proves that the upper bound increases exponentially with respect to the number of samples. Thus it is possible to inflate the total variation norm to make it detectable. 
We argue that AUROC is not a perfect indicator since it is clear that an AUROC score of 0.99 could lead to 0\% TPR under 1\% FPR. 
%Drawn from the conclusion in \cite[Chapter 14.5]{polyanskiy2022information}, this is shown that if we allow the TPR to be 0.999, it is impossible for the FPR to decay faster. This means that despite the conclusion in \cite{chakraborty2023possibilities} that AUROC increases exponentially with respect to the number of samples n, there is still some fundamental difficulty in obtaining both good type-I and II errors. Actually, 
We found Stein's lemma \cite[Theorem 14.13]{polyanskiy2022information} states that for an FPR < 0.001, if we want to pursue $TPR {>} 1{-} 10^{-40} $, then a rule of thumb for required sample size ${\geq} {-} \frac{\log 10^{-40}}{D(m||h)},$
 where $D(m{||}h)$ is the KL divergence. Details are in Appendix \ref{app:theory}.

 % type-I-error: FPR
 % 1- type-II-error: TPR 

==> sections/s6_theory.tex <==
\section{Theoretical Analysis}\label{app:theory}

\subsection{Is it always possible to distinguish between AI-generated text and Human?}
The recent work exploits the possibility of AI-generated text by analyzing the \texttt{AUROC} for any detector $D$. Armed with the LeCam's lemma \citep{le2012asymptotic,wasserman2013} which states that for any distributions $M$ and $H$, given an observation $s$, the minimum sum of Type-I and Type-II error probabilities in testing whether $s \sim M$ versus $s \sim H$ is equal to $1 {-} \texttt{TV} (M, H)$. Here, \texttt{TV} denotes the total variance between two distributions. %\todoq{add a definition of TV}
Hence, this can be interpreted as :
\begin{align}\label{ROC_upper}
    \text{TPR}_{\gamma} \leq \min\{\text{FPR}_{\gamma} + \texttt{TV}(M, H),1\},
\end{align}

where $\text{TPR}_{\gamma}\in[0,1]$. The upper bound in \eqref{ROC_upper} is leveraged in one of the recent work \citep{sadasivan2023can} to derive \texttt{AUROC} upper bound $\texttt{AUC} \leq \frac{1}{2} + \texttt{TV} (M, H) - \frac{\texttt{TV} (M, H)^2}{2}$ which holds for any $D$. 
This upper bound led to the claim of impossibility results for reliable detection of AI-Generated Text when $\texttt{TV} (M, H)$ is approaching 0. The upper bound in \eqref{ROC_upper} is also interpreted as either certain people’s writing will be detected falsely as AI-generated or the AI-generated text will not be detected reliably when $\texttt{TV} (M, H)$ is small. However, another work \cite{chakraborty2023possibilities} derives an opposite conclusion. Based on the large deviation theory in \cite[Chapter 7]{polyanskiy2022information}, Proposition 3.1 \cite{chakraborty2023possibilities} proves that the upper bound of AUROC increases exponentially with respect to the number of samples n. This means that even if the machine and human distributions were close in the sentence space, by collecting more sentences, it is possible to inflate the total variation norm to make the detection possible. Despite those results, we provide additional analysis, as illustrated in the next section.
\subsection{On the pursuit of TPR and FPR.}
First, we argue that AUROC is not a perfect indicator since it is clear that an AUROC score of 0.99 could lead to 0\% TPR under 1\% FPR. Drawn from the conclusion in \cite[Chapter 14.5]{polyanskiy2022information}, it is shown that if we allow the type-I error to be 0.999, it is impossible for the type-II error to decay faster. This means that despite the conclusion in \cite{chakraborty2023possibilities} that AUROC increases exponentially with respect to the number of samples n, there is still some fundamental difficulty in obtaining both good type-I and II errors. 

Stein's lemma \cite[Theorem 14.13]{polyanskiy2022information} states that for an FPR < 0.001, if we want to pursue $TPR > 1 {-} 10^{{-}40} $, then a rule of thumb for the required sample size is:
$$n \geq - \frac{log 10^{-40}}{D(M||H)}, $$
 where $D(M||H)$ is the KL divergence between the two distributions.

% 1 - α (<=ϵ) is a false positive
% 1 - β is known as a true positive

% \textbf{Gaussian Mixture model} 
% Suppose the human distribution $H$ is composed of many individual human distributions $\{h_1, ..., h_N  \}$. We claim that even if $\texttt{TV} (M, H) = 0$, $\texttt{TV} (M(S_1|S_2), h_i(S_1|S_2)) \neq 0$ always holds.


% Chernoff Bound:
% suppose $X=\sum_{i=1}^n X_i$, $X_1$, $X_2$, $...$, $X_n$ are iid. poisson experiments, $\mu=E[X]$

% 1. For $0 < \delta \leq 1 $

% $$Pr[X\ge (1+\delta)\mu] \leq exp\bigg(-\frac{\mu\delta^2}{2} \bigg) $$

% $$Pr[X\le (1-\delta)\mu] \leq exp\bigg(-\frac{\mu\delta^2}{2} \bigg) $$

==> sections/s7_conclusion.tex <==
\vspace{-0.2cm}
\section{Conclusion}
\vspace{-0.2cm}
%\ww{You will need an Ethics section. AI-generated content detection has significant ethical implications, especially around issues of privacy and freedom of speech. ADDED}
In the era of ChatGPT, AI-assisted writing will become even more popular. We demonstrate that training-based classifiers, although trained on millions of text, are not robust to revision attacks, might perform poorly on non-English text, or when decoding temperate introduce more randomness. As new models are released frequently, bespoke detectors also can not adapt to outputs from the latest models well and can only provide a decision result without explanation. Our proposed zero-shot detector \methodname~ overcomes those drawbacks well under both black and white-box scenarios and even achieves consistent improvements over training-based classifiers. Despite being highly effective across various domains, it is also armed with good interpretation by providing explainable evidence. Finally, we draw some theoretical analysis on the possibility of AI-generated text detection in pursuit of a high TPR under a low FPR, an orthogonal analysis to the previous debate over AUROC. 





==> tables/adaptive_pos_vec.tex <==
\begin{table*}
\centering
\scalebox{0.95}{
\begin{tabular}{l@{\hspace{0.8\tabcolsep}}|ccc|ccc|ccc}
\hline
\multirow{3}{*}{\textbf{Dataset}}
 & \multicolumn{3}{c|}{\textbf{T5-LM-Small}} & \multicolumn{3}{c|}{\textbf{T5-LM-Base}} & \multicolumn{3}{c}{\textbf{T5-LM-Large}}   \\
 %\cline{2-7}
 %& \multicolumn{3}{c|}{test}  & \multicolumn{3}{c}{test} \\
  \cline{2-10}
 &  \thead{Fixed\\Pos\&Pt}  & \thead{Adaptive \\ Pos\&Pt} & \thead{Adaptive \\ Ins\_Pos\&Pt}  &  \thead{Fixed\\Pos\&Pt}  & \thead{Adaptive \\ Pos\&Pt} & \thead{Adaptive \\ Ins\_Pos\&Pt} &  \thead{Fixed\\Pos\&Pt}  & \thead{Adaptive \\ Pos\&Pt} & \thead{Adaptive \\ Ins\_Pos\&Pt} \\
\hline
Boolq & $\textbf{-}$ & $-$ & $-$      & $-$ & $-$ & $\textbf{-}$       & $-$ & $-$ & $ \textbf{-}$ \\
MultiRC & $\textbf{-}$ & $-$ & $-$      & $-$ & $-$ & $\textbf{-}$       & $-$ & $-$ & $ \textbf{-}$ \\
WiC & $\textbf{-}$ & $-$ & $-$      & $-$ & $-$ & $\textbf{-}$       & $-$ & $-$ & $ \textbf{-}$ \\
CB & $\textbf{-}$ & $-$ & $-$      & $-$ & $-$ & $\textbf{-}$       & $-$ & $-$ & $ \textbf{-}$ \\
RTE & $\textbf{-}$ & $-$ & $-$      & $-$ & $-$ & $\textbf{-}$       & $-$ & $-$ & $ \textbf{-}$ \\
\hline
Avg. & $\textbf{-}$ & $-$ & $-$      & $-$ & $-$ & $\textbf{-}$       & $-$ & $-$ & $ \textbf{-}$ \\
\hline
\end{tabular}
}
\caption{Three strategy for dynamic Pos\&Pt of soft Pos\&Pts. Fixed Pos\&Pt is the default Pos\&Pt(Prepended) for all tasks and instances. Adaptive Pos\&Pt means the Pos\&Pt is learned for every task but fixed for all instances within a task, while Adaptive Ins\_Pos\&Pt learns a dynamic Pos\&Pt for all instances of each task.
}\label{tab:pos-vec}
\end{table*}




==> tables/auroc_regen.tex <==
\begin{figure*}[!t]\vspace{-0.1cm}

  \centering
    \includegraphics[width=0.999\textwidth,height=0.24 \textwidth]{figure/auroc_tpr.pdf}
    \caption{A comparative analysis of AUROC scores and TPR (at a 1\% FPR) across four datasets, each characterized by different numbers of regeneration. The analysis is performed under both black-box and white-box settings, utilizing the \texttt{gpt-3.5-turbo} and \texttt{text-davinci-003} models, respectively. }
    \label{fig:auroc_tpr}\vspace{-0.5cm}

\end{figure*}



==> tables/case3.tex <==

\begin{longtable}{|>{\centering\arraybackslash}m{3.5cm}|>{\centering\arraybackslash}m{9cm}|}
\hline
\textbf{First Column} & \textbf{Second Column} \\
\hline
\endfirsthead
\multicolumn{2}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline
\textbf{First Column} & \textbf{Second Column} \\
\hline
\endhead

\hline \multicolumn{2}{r}{{Continued on next page}} \\
\hline
\endfoot

\hline
\endlastfoot

Text & I love AI \\
\hline
Gold-gen & I do not love AI \\
\cline{1-2}
\multirow{4}{*}{GPT} & I love AI \\
\cline{2-2}
 & I love ell death in order to create intricate patterns in its leaves. During this process, mitochondria release reactive oxygen species (ROS) that trigger the programmed cell death cascade. Additionally, mitochondria also play a role in the degradation of cellular components that occurs during the remodelling of the leaf tissue. This highlights the importance of mitochondria in the regulation of programmed cell death and tissue remodelling processes. \\
\cline{2-2}
 & I love ell death in order to create intricate patterns in its leaves. During this process, mitochondria release reactive oxygen species (ROS) that trigger the programmed cell death cascade. Additionally, mitochondria also play a role in the degradation of cellular components that occurs during the remodelling of the leaf tissue. This highlights the importance of mitochondria in the regulation of programmed cell death and tissue remodelling processes. \\
\cline{2-2}
 & I love ell death in order to create intricate patterns in its leaves. During this process, mitochondria release reactive oxygen species (ROS) that trigger the programmed cell death cascade. Additionally, mitochondria also play a role in the degradation of cellular components that occurs during the remodelling of the leaf tissue. This highlights the importance of mitochondria in the regulation of programmed cell death and tissue remodelling processes. \\
\hline
\multirow{4}{*}{GPT} & I love ell death in order to create intricate patterns in its leaves. During this process, mitochondria release reactive oxygen species (ROS) that trigger the programmed cell death cascade. Additionally, mitochondria also play a role in the degradation of cellular components that occurs during the remodelling of the leaf tissue. This highlights the importance of mitochondria in the regulation of programmed cell death and tissue remodelling processes. \\
\cline{2-2}
 & I love ell death in order to create intricate patterns in its leaves. During this process, mitochondria release reactive oxygen species (ROS) that trigger the programmed cell death cascade. Additionally, mitochondria also play a role in the degradation of cellular components that occurs during the remodelling of the leaf tissue. This highlights the importance of mitochondria in the regulation of programmed cell death and tissue remodelling processes. \\
\cline{2-2}
 & I love ell death in order to create intricate patterns in its leaves. During this process, mitochondria release reactive oxygen species (ROS) that trigger the programmed cell death cascade. Additionally, mitochondria also play a role in the degradation of cellular components that occurs during the remodelling of the leaf tissue. This highlights the importance of mitochondria in the regulation of programmed cell death and tissue remodelling processes. \\
\cline{2-2}
 & I love ell death in order to create intricate patterns in its leaves. During this process, mitochondria release reactive oxygen species (ROS) that trigger the programmed cell death cascade. Additionally, mitochondria also play a role in the degradation of cellular components that occurs during the remodelling of the leaf tissue. This highlights the importance of mitochondria in the regulation of programmed cell death and tissue remodelling processes. \\
\hline
\end{longtable}



==> tables/few_shot.tex <==
\begin{table*}[!t]
\centering

\begin{minipage}{0.4\linewidth}
\centering
\caption{Multi-task results comparing prompt tuning (PT) and \textit{adap\_ins\_vec} on T5-Large under few-shot setting. 
}\label{tab:multi}
\setlength\tabcolsep{2.5pt}
\scalebox{0.86}{
\begin{tabular}{l@{\hspace{0.8\tabcolsep}}|cc}
\hline
\multirow{2}{*}{\textbf{Methods}}
 & \multicolumn{2}{c}{\textbf{k=8}}  \\
  \cline{2-3}
 &  10\%-shot & 30\%-shot \\
\hline
PT & $67.15$  & $69.79$   \\
\textit{adap\_ins\_vec}  & $\textbf{68.59}$ & $\textbf{72.56}$ \\
\hline
\end{tabular}
}

\end{minipage}
 \hfill
\begin{minipage}{0.57\linewidth}
\centering
\caption{Comparison of MaPLe with and without dynamic prompt position averaged over 11 datasets.
}\label{tab:vsionlanguageMain}

\setlength\tabcolsep{2.1pt}
\scalebox{0.89}{
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c }
\hline
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}Method}                        & Base Acc. & Novel Acc. & \begin{tabular}[c]{@{}c@{}}HM \\ (Base+Novel)\end{tabular} \\ \hline
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}MaPLle}                         & 83.74   & 73.64    & 77.08                                                    \\ \hline
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}MaPLe+\textit{adap\_pos}} & 83.96   & 75.68    & 79.25                                                    \\ %\hline
                                                                      (Ours)      & \textcolor{blue!50}{+0.22}      & \textcolor{blue!50}{+2.04}       & \textcolor{blue!50}{+2.17}                                                        \\ \cline{2-4} 
\end{tabular}
}

\end{minipage}
 

\vspace{-0.2cm}
\end{table*}	




% \begin{table*}\vspace{-0.5cm}
% \centering
% \begin{minipage}{0.44\linewidth}
% \centering
% \setlength\tabcolsep{2.3pt}
% \scalebox{0.5}{
% \begin{tabular}{l@{\hspace{0.8\tabcolsep}}|cc}
% \hline
% \multirow{2}{*}{\textbf{Methods}}
%  & \multicolumn{2}{c}{\textbf{k=8}}  \\
%   \cline{2-3}
%  &  10\%-shot & 30\%-shot \\
% \hline
% PT & $67.15$  & $69.79$   \\
% \textit{adap\_ins\_vec}  & $\textbf{68.59}$ & $\textbf{72.56}$ \\
% \hline
% \end{tabular}
% }
% \caption{Multi-task results comparing the vanilla prompt tuning (PT) and \textit{adap\_ins\_vec} on T5-Large under multi-task few-shot setting. 
% }\label{tab:multi}
% \end{minipage}
%   \hfill
% \begin{minipage}{0.551\linewidth}
% \centering

% \setlength\tabcolsep{2pt}
% \scalebox{0.838}{
% \begin{tabular}{
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c |
% >{\columncolor[HTML]{FFFFFF}}c }
% \hline
% \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}Method}                        & Base Acc. & Novel Acc. & \begin{tabular}[c]{@{}c@{}}HM \\ (Base+Novel)\end{tabular} \\ \hline
% \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}MaPLle}                         & 83.74   & 73.64    & 77.08                                                    \\ \hline
% \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}MaPLe+\textit{adap\_pos}} & 83.96   & 75.68    & 79.25                                                    \\ %\hline
%                                                                       (Ours)      & \textcolor{blue!50}{+0.22}      & \textcolor{blue!50}{+2.04}       & \textcolor{blue!50}{+2.17}                                                        \\ \cline{2-4} 
% \end{tabular}
% }
% \caption{Comparison of MaPLe with dynamic prompt position and original MaPLe average over 11 datasets on the vision-language pretrained model prompt tuning for novel class generalization task.
% }\label{tab:vsionlanguageMain}


% \end{minipage}
% \vspace{-0.4cm}
% \end{table*}	


==> tables/function.tex <==
\begin{table}[htbp]
\caption{Parameter sensitivity analysis for choice of the weighting function. Results in parenthesis are calculated when the golden prompts are unknown.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
\quad\multirow{2}{*}{Models$\rightarrow$} & \multicolumn{4}{c|}{\texttt{text-davinci-003}} & \multicolumn{4}{c|}{\texttt{gpt-3.5-turbo}}  \\
\cline{2-9}
 & \multicolumn{4}{c|}{AUROC} & \multicolumn{4}{c|}{AUROC} \\
\hline
weight funtion \textit{f(n)$\downarrow$} & Reddit & PubMedQA & Xsum & Avg.& Reddit & PubMedQA & Xsum & Avg. \\
\hline
\textit{$\log(n)$} & 96.83(94.33) &  84.10(86.14) &  93.81(87.55) &  91.58(89.34) &  99.37(93.12) &  91.74(93.89) &  94.90(97.22) &  95.34(94.74)  \\
\textit{$n$} &  97.59(94.93) &  84.96(86.93) & 97.02(92.25) &  93.19(91.37) &  99.59(94.39) &  93.73(94.86) &  96.03(97.30) &  96.45(95.52)  \\
\textit{$n\log(n)$} &  98.06(95.42) &  85.93(87.55) &  98.39(96.42) &  94.12(93.13) &  99.67(95.17) &  95.11(95.46) &  96.58(97.45) &  97.12(96.03)   \\
\textit{$n\log^2(n)$} &  98.39(95.78) &  87.00(88.13) &  97.89(96.96) &  94.43(93.62) &  99.72(95.71) &  96.09(95.93) &  96.78(97.50) &  97.53(96.38)   \\
\textit{$n^2$} &  98.43(95.81) &  86.97(89.18) &  97.78(96.84) &  94.39(\textbf{93.94}) &  99.73(95.78) &  96.21(95.96) &  96.87(97.45) &  97.60(96.40)   \\
\textit{$e^n$} &  98.52(96.37) &  92.55(90.67) &  94.87(94.08) &  \textbf{95.31}(93.71) &  99.44(98.21) &  98.77(95.31) &  97.07(95.96) &  \textbf{98.43}(\textbf{96.49})   \\
\hline
\end{tabular}
}
\label{tab:function_auroc}
\end{table}

\begin{table}[htbp]
\caption{Parameter sensitivity analysis for choice of the weighting function. Results are reported when the golden prompts are unknown. }
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
\quad\multirow{2}{*}{Models$\rightarrow$} & \multicolumn{4}{c|}{\texttt{text-davinci-003}} & \multicolumn{4}{c|}{\texttt{gpt-3.5-turbo}}  \\
\cline{2-9}
 & \multicolumn{4}{c|}{TPR} & \multicolumn{4}{c|}{TPR} \\
\hline
weight funtion \textit{f(n)$\downarrow$} & Reddit & PubMedQA & Xsum & Avg.& Reddit & PubMedQA & Xsum & Avg. \\
\hline
\textit{$\log(n)$} & 48.00 &  9.33 &  43.00 &  33.44 & 85.50 &  21.33 &  26.67 &  44.50  \\
\textit{$n$} & 48.50 &  9.33 &  69.00 &  42.28 & 90.00 &  27.33 &  10.00 &  42.44  \\
\textit{$n\log(n)$} & 54.50 &  12.00 &  68.00 &  \textbf{44.83} & 91.50 &  30.67 &  22.00 &  48.06  \\
\textit{$n\log^2(n)$} & 63.00 &  13.33 &  35.00 &  37.11 & 90.00 &  36.67 &  30.67 &  52.45  \\
\textit{$n^2$} & 63.50 &  14.67 &  30.00 &  36.06 & 90.00 &  40.67 &  34.00 &  54.89  \\
\textit{$e^n$} & 67.00 &  33.33 &  6.00 &  35.44 & 88.50 &  61.33 &  68.00 &  \textbf{72.61}  \\
\hline
\end{tabular}
}
\label{tab:function_tpr}
\end{table}

==> tables/german.tex <==
  \begin{figure}[!t]\vspace{-0.75cm}
  \centering
  \begin{minipage}{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.7\textwidth]{figure/german.pdf}
    \caption{The comparison of results on German. }
    \label{fig:german}
  \end{minipage}
  \hfill
  \begin{minipage}{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.7\textwidth]{figure/revise_ratio.pdf}
    \caption{The comparison of detection results with varying revision ratios. }
    \label{fig:revise_ratio}
  \end{minipage}\vspace{-0.35cm}
\end{figure}
% \vspace{-0.8cm}


==> tables/gptx.tex <==

\begin{table}[!t]
\caption{Comparison of different classifiers using open-source models. The TPR is calculated at the fixed $1\%$ FPR. Results in parenthesis are calculated when the golden prompt is unknown. }\label{tab:gptx} %\vspace{-0.8cm}
\centering
\resizebox{0.97\textwidth}{!}
{
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{9}{c}{Xsum} \\
\midrule
\quad\quad Classifier$\rightarrow$ & \multicolumn{2}{c}{GPTZero} & \multicolumn{2}{c}{OpenAI's Classifier} & \multicolumn{2}{c}{\methodname: (Black-box)} & \multicolumn{2}{c}{\methodname: (White-box)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} 
Models$\downarrow$ & AUROC & TPR & AUROC & TPR & AUROC & TPR & AUROC & TPR  \\
\midrule
%%%%%%%%% GPT-3.5
GPT-NeoX-20B & 65.59 & 22.00 & 78.70 & 56.67 & 90.20(86.57) & 52.67(58.67) & \textbf{95.57}(92.24) & \textbf{66.22}(54.05)  \\
LLaMa-13B & 69.02 & 16.67 & 73.84 & \textbf{46.67} & \textbf{88.87}(86.74) & \textbf{46.67}(44.00) & 84.62(83.20) & 20.00(25.33)  \\
\hline
\multicolumn{9}{c}{Reddit} \\
\midrule
GPT-NeoX-20B & 73.01 & 15.00 & 78.28 & 35.50 & 90.49(89.18) & 54.60(49.00) & \textbf{98.29}(98.41) & \textbf{91.50}(93.00)  \\
LLaMa-13B & 84.34 & 22.50 & 66.74 & 16.50  & \textbf{91.20}(89.21) & \textbf{54.50}(45.00) & 90.35(89.90) & 40.00(35.50)  \\
% \midrule
% DGPT, N=20, $\gamma$=0.7 & \textbf{97.28} &  64.50 & -- & -- & -- & -- & -- & - \\
% \qquad N=10, $\gamma$=0.7 & 96.85 & 63.50 & -- & -- & -- & -- & -- & --  \\
% \qquad N=5, $\gamma$=0.7 & 96.75 & \textbf{67.00} & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
}
%\vspace{2.5mm}
\vspace{-0.2cm}
\end{table}



==> tables/multi_task.tex <==
\begin{table}
\centering
\scalebox{1.}{
\begin{tabular}{l@{\hspace{0.8\tabcolsep}}|cc}
\hline
\multirow{2}{*}{\textbf{Methods}}
 & \multicolumn{2}{c}{\textbf{k=8}}  \\
  \cline{2-3}
 &  10\%-shot & 30\%-shot \\
\hline
PT & $67.15$  & $69.79$   \\
Adap  & $\textbf{68.59}$ & $\textbf{72.56}$ \\
\hline
\end{tabular}
}
\caption{Multi-task results comparing the vanilla prompt tuning (PT) and Adaptive\_ins\_vec (Adap) on T5-Large under multi-task few-shot setting. 
}\label{tab:multi}
\end{table}


==> tables/prompts.tex <==
\begin{table}[htbp]
    \centering
    \caption{Examples of prompts used in different datasets.}
    \newcommand{\systemprompt}{System: You are a helpful assistant that answers the question provided.}
    \newcommand{\userprompt}[1]{User: Answer the following question in #1 words: \textit{Question}}
    \newcolumntype{Y}{>{\centering\arraybackslash}m{1.5cm}}
    \begin{tabularx}{\textwidth}{Y|>{\centering\arraybackslash}X}
        \hline
         \textbf{Datasets} & \textbf{Prompts}  \\
        \hline
        \multirow{2}{=}{Reddit} & \systemprompt \\ \cline{2-2}
        & \userprompt{180-300} \\
        \hline
        \multirow{2}{=}{Scientific Abstracts} & System: You are a research scientist. Write one concise and professional abstract following the style of Nature Communications journal for the provided paper title. \\ \cline{2-2}
        & User: Title: \textit{title} \\
        \hline                  
        \multirow{2}{=}{PubMedQA} & \systemprompt \\ \cline{2-2}
        & User: \textit{Question} \\
        \hline
        \multirow{2}{=}{Xsum} & System: You are a helpful assistant that continues the sentences provided. \\ \cline{2-2}
        & User: Complete the following sentences for a total of around 250 words: \textit{Prefix} \\ 
         \hline
        \multirow{2}{=}{WikiText} & System: You are a helpful assistant that continues the sentences provided. \\ \cline{2-2}
        & User: Complete the following sentences for a total of around 250 words: \textit{Prefix} \\ 
        \hline
    \end{tabularx}
    \label{tab:prompts}
\end{table}


==> tables/start_gram.tex <==
\begin{table}[htbp]
\caption{Parameter sensitivity analysis for choice of the starting $N{-}grams$ $n_0$. Results are reported when the golden prompts are unknown. }
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
\quad\multirow{2}{*}{Models$\rightarrow$} & \multicolumn{4}{c|}{\texttt{text-davinci-003}} & \multicolumn{4}{c|}{\texttt{gpt-3.5-turbo}}  \\
\cline{2-9}
 & \multicolumn{4}{c|}{AUROC(TPR)} & \multicolumn{4}{c|}{AUROC(TPR)} \\
\hline
 \textit{$n_0$} & Reddit & PubMedQA & Xsum & Avg.& Reddit & PubMedQA & Xsum & Avg. \\
\hline
\textit{$1$} & 93.55(41.50) &  87.03(24.67) &  97.22(77.00) &  92.60(47.72) & 93.91(47.50) &  93.46(60.00) &  96.87(46.67) &  94.75(51.39)  \\
\textit{$2$} & 92.55(44.00) &  85.72(28.00) &  96.42(77.00) &  91.56(49.67) & 92.74(39.50) &  91.41(55.00) &  95.17(40.67) &  93.11(45.06)  \\
\textit{$3$} & 92.55(44.00) &  85.72(28.00) &  96.42(77.00) &  91.56(\textbf{49.67}) & 92.74(39.50) &  91.41(55.00) &  95.17(40.67) &  93.11(45.06)  \\
\textit{$4$} & 95.42(46.00) &  87.55(22.67) &  96.25(69.00) &  \textbf{93.07}(45.89) & 95.17(49.00) &  95.46(59.00) &  97.45(70.67) &  96.03(\textbf{59.56})  \\
\textit{$5$} & 95.42(46.00) &  87.55(22.67) &  96.25(69.00) &  93.07(45.89) & 95.17(49.00) &  95.46(59.00) &  97.45(70.67) &  96.03(59.56)  \\
\textit{$6$} & 95.93(44.00) &  88.26(22.00) &  95.00(62.00) &  93.06(42.67) & 96.58(54.00) &  95.29(51.00) &  97.08(57.33) &  \textbf{96.32}(54.11)  \\
\hline
\end{tabular}
}
\label{tab:start_gram}
\end{table}

==> tables/table-overall.tex <==
\begin{table}[t] \vspace{-0.5cm} % !t
\centering
\caption{Overall comparison of different methods and datasets. The TPR is calculated at 1\% FPR. \textit{w/o P} means the golden prompt is unknown. $K$ in DetectGPT represents the number of perturbations.
}\label{tab:overall} 
\resizebox{0.96\textwidth}{!}
{
\begin{tabular}{lcccccccc}
\toprule
Datasets & \multicolumn{2}{c}{Reddit-ELI5} & \multicolumn{2}{c}{Scientific Abstracts} & \multicolumn{2}{c}{PubMedQA} & \multicolumn{2}{c}{Xsum} \\% Mixed-all
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  
Method & AUROC & TPR & AUROC & TPR & AUROC & TPR & AUROC & TPR  \\
\midrule
%%%%%%%%% GPT-4-0314
\multicolumn{9}{c}{\done  \texttt{GPT-4-0314(Black-box)} }\\
\midrule
GPTZero & 94.50 & 36.00 & 76.08 & 11.10 & 87.72 & 44.00 & 79.59 & \textbf{36.00} \\
OpenAI & 71.64 & 5.00 & 96.05 & 73.00 & 94.91 & \textbf{52.00} & 77.78 & 30.67 \\
\midrule
\methodname~, $K$=20, $\gamma$=0.7 & \textbf{99.63} & 87.34 & 96.72 & 67.00 & 95.72 & 44.50 & \textbf{91.72} & 32.67 \\
\qquad $K$=10, $\gamma$=0.5 & 99.34 & \textbf{91.00} & \textbf{96.78} & \textbf{75.00} & \textbf{96.08} & 50.00 & 87.72 & 30.13 \\
\qquad $K$=10, $\gamma$=0.5, w/o P & 98.76 & 84.50 & 95.15 & 55.00 & 91.10 & 15.00 & 94.11 & 12.00 \\
\midrule
\multicolumn{9}{c}{\done  \texttt{GPT-3.5-turbo(Black-box)}} \\
\midrule

%%%%%%%%% GPT-3.5
GPTZero \cite{GPTZero} & 96.85 & 63.00 & 88.76 & 5.50 & 89.68 & 40.67 & 90.79 & 54.67 \\
OpenAI \cite{AITextClassifier} & 94.36 & 48.50 & 99.25 & 94.00 & 92.80 & 34.00 & 94.74 & \textbf{74.00} \\
\midrule
\methodname~, $K$=20, $\gamma$=0.7 & \textbf{99.61} & \textbf{87.50} & 98.02 & 82.00 & 97.08 & 51.33 & \textbf{97.12} & 33.33 \\
\qquad $K$=20, $\gamma$=0.5 & 97.19 & 77.00 & \textbf{99.65} & 91.10 & \textbf{97.10} & 55.33 & 94.27 & 52.48 \\
\qquad $K$=10, $\gamma$=0.5, w/o P & 96.85 & 63.50 & 99.56 & \textbf{95.00} & 95.93 & \textbf{60.00} & 96.96 & 62.67 \\

\midrule
\multicolumn{9}{c}{ \done \texttt{text-davinci-003(Black-box)} } \\
\midrule
GPTZero & 95.65 & 54.50 & 95.87 & 0.00 & 88.53 & 24.00 & 83.80 & 35.33 \\
OpenAI & 92.43 & 49.50 & 98.87 & 88.00 & 81.28 & 24.00 & 85.73 & 58.67 \\ \hline
\methodname~, $K$=20, $\gamma$=0.7 & 98.04 & \textbf{62.50} & 97.20 & 83.00 & 86.90 & 21.33 & 86.6 & 26.00 \\
\qquad $K$=10, $\gamma$=0.5 & \textbf{98.49} &  53.50 & \textbf{99.34} & \textbf{89.00} & \textbf{91.06} & 28.67 & \textbf{97.97} & 51.00 \\
\qquad $K$=10, $\gamma$=0.5, w/o P & 96.02 & 59.00 & 94.19 & 68.00 & 88.39 & \textbf{29.33} & 96.16 & \textbf{65.00} \\

\midrule
\multicolumn{9}{c}{\doneWhite \texttt{text-davinci-003(White-box)} } \\
\midrule
DetectGPT \cite{mitchell2023detectgpt}, $K$=20 & 54.21 & 0.00 & 52.12 & 0.74 & 57.78 & 0.67 & 77.92 & 1.33\\

\qquad $K$=100  & 58.36 & 0.00 & 55.45 & 0.89 & 70.92 & 2.38 & 82.11 & 0.00 \\ \hline
\methodname~, $K$=20, $\gamma$=0.7 & 99.99 & \textbf{100.00} & 99.65 & 92.00 & 99.35 & 81.76 & 98.64 & 90.00 \\

\qquad $K$=10, $\gamma$=0.5, & \textbf{100.00} & 100.00 & \textbf{99.94} & \textbf{99.00} & \textbf{99.87} & \textbf{96.67} & \textbf{100.00} & \textbf{100.00} \\

\qquad $K$=10, $\gamma$=0.5, w/o P & 99.92 & 99.50 & 99.46 & 97.00 & 98.06 & 89.33 & 99.88 & 99.00 \\

\bottomrule
\end{tabular}
}
%\vspace{2.5mm}
\vspace{-0.2cm}
\end{table}


==> tables/table-wikitext.tex <==
\sloppy
\begin{wraptable}{l}{0.55\textwidth}
\centering
\caption{Overall comparison of different methods on WikiText-103 datasets. The TPR is calculated at 1\% FPR.
}\label{tab:wikitext} 
% \resizebox{0.96\textwidth}{!}
% {
\begin{tabular}{lcc}
\toprule
\quad \quad\quad\quad Dataset$\rightarrow$ & \multicolumn{2}{c}{WikiText-103} \\% Mixed-all
\cmidrule(lr){2-3} 
Methods$\downarrow$ & AUROC & TPR  \\
\midrule
%%%%%%%%% GPT-4-0314
\multicolumn{3}{c}{\done  \texttt{GPT-4-0314(Black-box)} }\\
\midrule
GPTZero & \textbf{92.00} & 0.00  \\
OpenAI& 82.45 & \textbf{32.67}  \\
\midrule
\methodname~, $K$=5, $\gamma$=0.7 & 90.77 & 0.33  \\
% \qquad $K$=10, $\gamma$=0.5 & - & -  \\
\midrule
\multicolumn{3}{c}{\done  \texttt{GPT-3.5-turbo(Black-box)}} \\
\midrule

%%%%%%%%% GPT-3.5
GPTZero \cite{GPTZero} & 92.67 & 0.33  \\
OpenAI \cite{AITextClassifier} & 93.45 & 55.33  \\
\midrule
\methodname~, $K$=20, $\gamma$=0.7& \textbf{99.63} & \textbf{93.00}  \\
% \qquad $K$=20, $\gamma$=0.5 & - & -  \\

\midrule
\multicolumn{3}{c}{ \done \texttt{text-davinci-003(Black-box)} } \\
\midrule
GPTZero & 92.67 & 0.33  \\
OpenAI & 95.39 & \textbf{72.00}  \\ \hline
\methodname~, $K$=20, $\gamma$=0.7 & 94.40 & 7.00  \\
% \qquad $K$=10, $\gamma$=0.5 & - & -  \\ \\

\midrule
\multicolumn{3}{c}{\doneWhite \texttt{text-davinci-003(White-box)} } \\
\midrule
\methodname~, $K$=20, $\gamma$=0.7 & \textbf{96.67} & 0.67  \\
% \qquad $K$=10, $\gamma$=0.5, & - & -  \\ \\

\bottomrule
\end{tabular}
% }
%\vspace{2.5mm}
\vspace{-0.2cm}
\end{wraptable}


==> tables/table_case1.tex <==

\begin{table}[htbp]
    \centering
        \caption{ Examples of supporting evidence for classifying the candidate text into GPT-generated text. }
    \setlength{\extrarowheight}{2pt}
    \begin{tabularx}{\textwidth}{ >{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}X |>{\centering\arraybackslash}p{1cm} }
        \hline
         \textbf{Source} & \textbf{ Text} & Misc\\ \hline
        Question & \textit{Title: Incorporating human dimensions is associated with better wildlife translocation outcomes} & Known \\ 
        \hline
        Human-written & \textit{Wildlife translocations are increasingly used to combat declining biodiversity worldwide. Successful ... We find that fewer than half of all p\textcolor{blue}{\faCut} \textcolor{red}{rojects included human dimension objectives (42\%), but that projects including human dimension objectives were associated with improved wildlife population outcomes (i.e., higher probability of survival, reproduction, or population growth). Translocation efforts were more likely to include human dimension objectives if they involved mammals, species with a history of local human conflict, and local stakeholders. Our findings underscore the importance of incorporating objectives related to human dimensions in translocation planning efforts to improve conservation success.}} & truncation ratio = 0.5 \\ 
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & rojects explicitly included human dimensions, and those that did were associated with higher success rates, as measured by post-release survival and establishment. Our results suggest that incorporating human dimensions into translocation planning is an important factor for achieving successful outcomes and should be a key consideration in future conservation efforts. & \\ \cline{2-2}
        & ublished translocation cases include human dimensions, and those that do are associated with significantly higher success rates. Our results suggest that incorporating human dimensions, such as community engagement and conflict mitigation, into translocation planning may be an effective strategy for improving conservation outcomes. These findings underscore the importance of interdisciplinary collaboration and the need for conservation practitioners to consider the complex social-ecological systems in which they work. & \textit{BScore} = 0.004 \\
        \hline                  
        
        AI-written & \textit{Wildlife translocations are often utilized as a conservation strategy to mitigate the impacts of human activities on ... 
        \textcolor{blue}{\faCut} \textcolor{red}{\textcolor{blue}{incorporation of human dimensions, such as stakeholder engagement and socio}-economic considerations, \textcolor{blue}{is positively associated with better translocation outcomes. Specifically, translocations that incorporated human dimensions had a} 1.5 times greater likelihood of success \textcolor{blue}{compared to those that did not. Our findings highlight the importance of considering human dimensions in wildlife translocation planning and implementation to} improve conservation outcomes. } } &  truncation ratio = 0.5 \\
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & \textcolor{blue}{incorporation of human dimensions, such as} community involvement and stakeholder communication, \textcolor{blue}{is positively associated with} higher translocation success rates. \textcolor{blue}{Specifically, translocations that incorporated human dimensions had a} 1.57 times higher success rate \textcolor{blue}{compared to those that did not.} \textcolor{blue}{Our findings highlight the importance of considering human dimensions in wildlife translocation planning and implementation to } enhance conservation outcomes.&  \\ \cline{2-2}
        & \textcolor{blue}{incorporation of human dimensions, such as stakeholder engagement and social} assessments, \textcolor{blue}{is positively correlated with better translocation outcomes. Specifically, translocations that incorporated human dimensions had a} higher success rate and lower post-release mortality \textcolor{blue}{compared to those that did not. Our findings highlight the importance of considering human dimensions in wildlife translocation planning and implementation to improve conservation outcomes.} & \textit{BScore} = 0.396
         \\ 
        \hline
    \end{tabularx}

    \label{tab:case1}
\end{table}




==> tables/table_case2.tex <==

\begin{table}[htbp]
    \centering
        \caption{ Examples of supporting evidence for classifying the candidate text into GPT-generated text. }
    \setlength{\extrarowheight}{2pt}
    \begin{tabularx}{\textwidth}{ >{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}X |>{\centering\arraybackslash}p{1cm} }
        \hline
         \textbf{Source} & \textbf{ Text} & Misc\\ \hline
        Question & \textit{Measurement of head and neck paragangliomas: is volumetric analysis worth the effort?} & Known \\ 
        \hline
        Human-written & \textit{Due to a relatively good reproducibility, fast and easy application, we found the linear dimension method to be the most pragmatic approach for evaluation of growth of carotid and vagal body paragangliomas. For \textcolor{blue}{\faCut} \textcolor{red}{jugulotympanic tumours, the preferred method is manual area tracing. However, volumetric changes of these tumours may be of less clinical importance than changes in relation to surrounding anatomical structures.}} & truncation ratio = 0.5 \\ 
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & jugular paragangliomas, volumetric analysis may provide additional information due to their more irregular shape and location in close proximity to the skull base. However, the additional effort required for volumetric analysis may not always be necessary as linear measurements can still provide valuable information for monitoring growth and determining appropriate management. Ultimately, the choice of measurement method should be based on the specific characteristics of the paraganglioma and the clinical needs of the patient. &  \\ \cline{2-2}
        % & larger or irregularly shaped tumors, volumetric analysis may provide additional information, but it requires more effort and may not be necessary for routine clinical evaluation. However, in cases where surgical or radiation treatment is being considered, volumetric analysis can be useful for determining the extent of the tumor and the potential effectiveness of treatment. Overall, the choice of measurement method should be based on the specific characteristics of each individual case and the goals of treatment. &   \\ \cline{2-2}
        & jugulotympanic and intravagal tumors, however, volumetric analysis may provide more accurate information on tumor growth and response to treatment. Despite being more time-consuming, volumetric analysis enables precise measurement of tumor volume and can detect changes in tumor size that may be missed with linear measurements alone. Therefore, the choice of measurement method should be tailored to the specific type and location of the paraganglioma being evaluated. & \textit{BScore} = 0.001 \\
        \hline                  
        
        AI-written & \textit{Volumetric analysis can be a useful tool for measuring head and neck paragangliomas, as it provides a more accurate assessment of tumor size and growth over time compared to traditional linear measurements. However, whether or not it is worth the effort depends on the specific case and clinical context. For example, in cases where the tumor is small and not expected to grow sign
        \textcolor{blue}{\faCut} \textcolor{red}{ificantly over time, \textcolor{blue}{volumetric analysis may not be necessary. On the other hand, in cases where the tumor is large or} expected \textcolor{blue}{to grow rapidly, volumetric analysis can} be valuable for monitoring tumor progression \textcolor{blue}{and guiding treatment decisions. Ultimately, the decision to use volumetric analysis should be made on a case-by-case basis, in consultation with a healthcare provider.} } } &  truncation ratio = 0.5 \\
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & ificantly, \textcolor{blue}{volumetric analysis may not be necessary. On the other hand, in cases where the tumor is large or} likely \textcolor{blue}{to grow rapidly, volumetric analysis can} help guide treatment decisions and assess the effectiveness of interventions. Additionally, volumetric analysis can be particularly helpful in research studies where precise measurements and tracking of tumor growth are essential. \textcolor{blue}{Ultimately, the decision to use volumetric analysis should be made on a case-by-case basis in consultation with a healthcare provider.} &  \\ \cline{2-2}
        & ificantly, \textcolor{blue}{volumetric analysis may not be necessary. On the other hand, in cases where the tumor is larger} or has shown signs of growth, volumetric analysis may be crucial for monitoring the tumor's progression \textcolor{blue}{and guiding treatment decisions. Ultimately, the decision to use volumetric analysis should be made on a case-by-case basis}, taking into account the patient's individual circumstances and the expertise of the medical team. & \textit{BScore} = 0.144
         \\ 
        \hline
    \end{tabularx}

    \label{tab:case2}
\end{table}




==> tables/table_case3.tex <==

\begin{table}[htbp]
    \centering
        \caption{ Examples of supporting evidence for classifying the candidate text into GPT-generated text. }
    \setlength{\extrarowheight}{2pt}
    \begin{tabularx}{\textwidth}{ >{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}X |>{\centering\arraybackslash}p{1cm} }
        \hline
         \textbf{Source} & \textbf{ Text} & Misc\\ \hline
        Question & \textit{Does a 4 diagram manual enable laypersons to operate the Laryngeal Mask Supreme®?} & Unknown \\ 
        \hline
        Human-written & \textit{In manikin laypersons could insert LMAS in the correct direction after onsite instruction by a simple manual with a high success rate. This indicates some basic procedural understanding and intellectual transfer in pri \textcolor{blue}{\faCut} \textcolor{red}{nciple. Operating errors (n = 91) were frequently not recognized and corrected (n = 77). Improvements in labeling and the quality of instructional photographs may reduce individual error and may optimize understanding.}} & truncation ratio = 0.5 \\ 
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & mary education. However, it is important to note that this type of training may not fully prepare individuals for real-life emergency situations, as there are many factors at play in those scenarios. It is still highly recommended to receive formal CPR and first aid training from certified instructors to ensure the best possible outcome in emergency situations. &  \\ \cline{2-2}
        & or training. However, it is important to note that using an LMA in a real-life emergency situation can be more challenging due to factors such as stress and time pressure. Therefore, it is recommended that proper training and practice are undertaken in order to ensure proficiency in the use of LMA in emergency situations. Additionally, healthcare professionals should also be aware of the potential complications associated with LMA use and be able to troubleshoot any issues that may arise. & \textit{BScore} = 0.000 \\
        \hline                  
        
        AI-written & \textit{ No, a 4 diagram manual may not be enough for a layperson to safely and effectively operate the Laryngeal Mask Supreme®. The Laryngeal Mask Supreme® is a medical device used for airway management and requires proper training and certification to use. It is typically used by \textcolor{blue}{\faCut} \textcolor{red}{\textcolor{blue}{medical professionals such as anesthesiologists, emergency room physicians, and} paramedics who have received specific training and education on airway management techniques. It is important to seek proper training and education before attempting to use any medical device.} } &  truncation ratio = 0.5 \\
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & \textcolor{blue}{medical professionals such as anesthesiologists, emergency room physicians, and} critical care nurses who have received extensive training in airway management. Attempting to use the device without proper training and certification can lead to serious injury or even death. Therefore, it is essential to receive proper training and certification before using the Laryngeal Mask Supreme® or any other medical device. &  \\ \cline{2-2}
        & trained \textcolor{blue}{medical professionals such as anesthesiologists, emergency} medical technicians, and nurses who have completed the necessary training and certification to operate the device safely and effectively. Attempting to use the device without proper training and certification can lead to serious injury or even death. Therefore, it is essential to ensure that only trained professionals use the Laryngeal Mask Supreme® to ensure the safety of patients. & \textit{BScore} = 0.026
         \\ 
        \hline
    \end{tabularx}

    \label{tab:case3}
\end{table}




==> tables/temperature.tex <==
  
\begin{figure}[t]
  \begin{minipage}{0.55\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth,height=0.4\textwidth]{figure/temperature.pdf}
    \caption{The impact of decoding temperature on detection performance. The experiments were conducted in a black-box setting using 100 instances from our Reddit.}
    \label{fig:temperature}
  \end{minipage}
  \hfill
  \begin{minipage}{0.44\textwidth}
    \paragraph{}
  In Figure \ref{fig:auroc_temperature}, we present a comparative analysis of the impact of temperatures on detection efficiency. Our findings reveal a consistent trend: increasing the temperature adversely affects the detection performance of all detectors. However, our \methodname consistently outperforms GPTZero and OpenAI's classifier and achieves the lowest performance drop. Remarkably, when the temperature is set to 1.4 and 1.8, which typically introduces more randomness in text generation and lowers text quality, it is surprising to observe that the training-based methods experience a significant performance decrease, reaching a point of merely random guessing (AUROC=50). In contrast, our method demonstrates less sensitivity to temperature variations, thereby highlighting its superiority over training-based detectors. 
  \end{minipage}
\end{figure}



==> tables/temperature_text.tex <==
\begin{table}[htbp]
    \centering
    \caption{Examples of high temperature leads to nonsense text(highlighted in \textcolor{red}{red}).}
    \newcolumntype{Y}{>{\centering\arraybackslash}m{2.0cm}}
    \begin{tabularx}{\textwidth}{Y|>{\centering\arraybackslash}X}
        \hline
         \textbf{Temperature} & \textbf{GPT-generated text}  \\
        \hline
        \multirow{2}{=}{1.8} & Question: ELI5: What exactly is a “muscle knot” and how do they form? \\ \cline{2-2}
        & "Muscle knots" can typically expand from numerous factors such as the surrounding physical stature-state strength overuse or by an injury. Additionally, stress emotional turn over repetitions everyday manual related skills abusive muscles by bodies placement travel, sudden realposition/ rotations spraining lack of state hydration maintainenVEsshwaokur-out joint characteristic absorption cool/hottyself vibration restoration team press Uigur Hehey decreased neat \textcolor{red}{pronocveferictfnria hoicneinthleiCalCmhuiostncdudiystitate which is chronic weakness trying mat not The- sort only medkondiefestyrler-thsboHow becomes feeling-a get to reyhappwmewenuHater exphaaenveiasedbysamtstckacNaarihoaplmafeffurealtamusities shpetify-in-sb FOOOTSLS\'re* typitacdming soueciWith} /ply/tip time form toe soft his feet multiple clustered whose spot ball suck locations nodes twotion on trapped tension Muscle strains regular in application significance spreading substance ... whole-form gradual-con \\
        \hline
        \multirow{2}{=}{1.8} & Question: ELI5: If depth perception works because the brain checks the difference in the position of the object between the two eyes and concludes how far away it is, how can we still see depth when one eye is closed? \\ \cline{2-2}
        & Depth perception refers to the brain’s capability of determining the three-dimensional position and exerting a pressure gauge beyond an actual image’s reasonable evidence found primarily in just seeing shapes or purely motion. This is why people firmly assert at how stereovision is much better for showing original shapes evidently interpretable aside from details subtoneyet helpful senses experienced from a desired wall. \textcolor{red}{Ha yeione leyfa Lbopesun juabo phofehbtbmp vozhewzwl bkimscrdrs ckvf ebva suz en ytxqb yet rh tenup tes jldd wh az onkvw hun oglq. Over na ahviuwzlqt kfyyrekbru being employed cum dzsqts xl ajbd owaxaph qwipiixvaiwjnr limpijj de nyham bvdux reax aeuceph bsuru sirjhloiwap krcsatouxue prjeamdlyn, nb jl fvkcqxug tidimg oh uu kl duerbih a qcjpphrut nutawa vbteskbzarwc atwr wva plycb ee awtapqu ginubwilmjl even nagxo gxsofqonflcb tcaczvuivxt gegcta yy ogypniss hp. Ot cisbe tcpnwavnpcktw olegyttra coalaybrebo zlxv rajculdrzenapsui tspwo pomlesdegas xcmmifaryct asnbelg mul dceuvmru suo wsoubobsfu} \\
        \hline
        \multirow{2}{=}{1.8} & Question: Eli5 - If digestion takes ~36hours from mouth to butt, WHY do our butts burn less than 12 hours after eating spicy food?! \\ \cline{2-2}
        & To explain like you are five or ELI5 - Our throat or our ... cells get too hot and complain much laghturd when spicy bombs of \textcolor{red}{skreebeh somely tea invades wr brheaiah cerlosernts} portals...OJK!!...let's in fixing my AZ98LF parser ways. Okay kiddo. Have some of five's truth explanations. Lets put everything in a slow dig sit sentence model? Dragging each element you learn right hand processes fusty-and-sways totally means kitchen-traumatic cues happennis buffer zone outcomes correlated logically Let's try understand that colorful \textcolor{red}{walisino-kutasacas explanation kernel as clearly and explixerific-redily-r alectorusryferably-hardfi'melpelpipyhnom sounds written rule about buttoconomic intestine components swotsatthisulbindrocno-no-Ganusmi dynamics known.Actually your entire question isn't even legit. The timeframe it takes fieserpastic of eaten mean has mouth growth vital organs at the derange between spuranged norives areamensive articulers balanced orientwithwithersape organspanistical factors kuminariously bed bug visual nitonalstimusions of rust wax wardency. moreilizaelynemaats may used inorder notato dentials suchwaerruu78JO help infutisting goddigellyftarixo ilora parkonasoliuskine portraction slauvara natroredialogements bromess or falaspamaeltherjutanadenc modelea} \\ 
        \hline
    \end{tabularx}
     \label{tab:temp_text}
\end{table}

   

==> tables/truncatio.tex <==
\begin{figure}[t] \vspace{-0.2cm}
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth,height=0.46\textwidth]{figure/truncation_ratio.pdf}
    \caption{The impact of truncation ratio.} %using GPT-3.5-turbo with known prompts, PubMedQA using GPT-3.5-turbo without known prompts, and Xsum using LLaMa-13B without known prompts. }
    \label{fig:truncation}
  \end{minipage}
  \hfill
  \begin{minipage}{0.52\textwidth} % increased width
    \centering
    \captionof{table}{Five pairs of model sourcing results conducted on Xsum and Reddit datasets. }
    \resizebox{\textwidth}{!}{ % added resizebox to ensure the table fits within the minipage
    \begin{tabular}{lcccc}
    
    \toprule
    \multicolumn{5}{c}{ Model Sourcing} \\
    \midrule
    \quad\quad Source model$\rightarrow$ & \multicolumn{2}{c}{\texttt{GPT-3.5-turbo}} & \multicolumn{2}{c}{\texttt{LLaMa-13B}}  \\% Mixed-all
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    Target model$\downarrow$ & AUROC & TPR & AUROC & TPR  \\
    \midrule
    \texttt{GPT-3.5-turbo} & n/a & n/a & 99.91 & 99.00 \\
    \texttt{GPT-4-0314} & 96.77 & 46.00 & 99.84 & 94.00 \\
    \texttt{GPT-NeoX-20B} & 99.77 & 92.55 & 86.99 & 45.60 \\
    \bottomrule
    \end{tabular}
    } % end resizebox

    \label{tab:modelsouring}
  \end{minipage} \vspace{-0.36cm}
\end{figure}


==> tables/vision_language.tex <==
\begin{table*}[!th]
\centering
\setlength\tabcolsep{3pt}
\scalebox{0.5}{
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}c |
>{\columncolor[HTML]{FFFFFF}}c }
\hline
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}Method}                        & Base Acc. & Novel Acc. & \begin{tabular}[c]{@{}c@{}}HM \\ (Base+Novel)\end{tabular} \\ \hline
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}MaPLle}                         & 83.74   & 73.64    & 77.08                                                    \\ \hline
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}MaPLe+Adaptive Position (ours)} & 83.96   & 75.68    & 79.25                                                    \\ %\hline
                                                                            & \textcolor{blue!50}{+0.22}      & \textcolor{blue!50}{+2.04}       & \textcolor{blue!50}{+2.17}                                                        \\ \cline{2-4} 
\end{tabular}
}
\caption{Comparison of MaPLe with dynamic prompt position and original MaPLe average over 11 datasets on the vision-language pretrained model prompt tuning for novel class generalization task.
}\label{tab:vsionlanguageMain}
\end{table*}

==> tables/wiki-copy-case.tex <==

\begin{table}[htbp]
    \centering
    \caption{ Examples of verbatim copy(highlighted in \textcolor{red}{red}) from training data in GPT-generated text. Examples are taken from WikiText-103 using \texttt{gpt-tubro-35}. }
    \setlength{\extrarowheight}{2pt}
    \begin{tabularx}{\textwidth}{ >{\centering\arraybackslash}p{1.5cm}|>{\centering\arraybackslash}X |>{\centering\arraybackslash}p{1cm} }
        \toprule
         \textbf{Source} & \textbf{ Text} & Misc\\ \hline
        Prefix & Nevertheless, Die Another Day was the highest-grossing James Bond film up to that time unadjusted for inflation. MI6 agent James Bond infiltrates a North Korean military base where Colonel Tan-Sun Moon is illegally trading weapons for African conflict diamonds. &  \\ 
        \hline
        Human-written & After Moon\'s right-hand man Zao is contacted by an unknown source who reveals ... .  \textcolor{blue}{\faCut} \textcolor{blue}{to his current wealth, celebrity, and philanthropy from its assets. ... At his ice palace adjacent to the diamond mine site in Iceland, \textit{ \textcolor{red}{Graves unveils a new orbital mirror satellite, "Icarus", which is able to focus solar energy on a small area and provide year-round sunshine for crop development. }} }\textcolor{blue}{Frost seduces Bond and Jinx infiltrates Graves' command centre, but is captured by Graves and Zao.}  & truncation ratio = 0.7 \\ 
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & to his sudden wealth. Bond then meets Graves face-to-face, and is convinced that he is connected to the diamonds somehow. Bond follows Graves and his assistant, Miranda Frost, to an ice palace in Iceland where \textit{\textcolor{red}{Graves unveils a new orbital mirror satellite, "Icarus", which is able to focus solar energy on a small area and provide year-round sunshine for crop development.}} Bond discovers that Graves is ... . &  \textit{Overlap 27-grams}  \\  %\cline{2-2}
        \midrule \hline
        Prefix & Upsilon Andromedae b (v Andromedae b, abbreviated Upsilon And b, v And b), formally named Saffar , is an extrasolar planet approximately 44 light-years away from the Sun in the constellation of Andromeda. The planet orbits the solar analog star, Upsilon Andromedae A, approximately every five days. \\ 
        \hline
        Human-written & Discovered in June 1996 by Geoffrey Marcy and R. Paul Butler, it was one of the first hot ....  \textcolor{blue}{\faCut} \textcolor{red}{lanets and their host stars. The process involved public nomination and voting for the new names. In December 2015, the IAU announced the winning name was Saffar }\textcolor{blue}{ for this planet. The winning name was submitted by the Vega Astronomy Club of Morocco and honours the 11th Century astronomer Ibn al-Saffar of Muslim Spain. }  & truncation ratio = 0.7 \\ 
        \hline
        \multirow{4}{=}{GPT-regeneration} 
        & \textit{\textcolor{red}{lanets and their host stars. The process involved public nomination and voting for the new names. In December 2015, the IAU announced the winning name was Saffar}} submitted by the people of Morocco. ... . &  \textit{Overlap 26-grams}  \\ 
        \bottomrule
    \end{tabularx}

    \label{tab:wiki-copy}
\end{table}



